NUSense: Robust Soft Optical Tactile Sensor

While most tactile sensors rely on measuring pressure, insights from continuum mechanics suggest that measuring shear strain provides critical information for tactile sensing. In this work, we introduce an optical tactile sensing principle based on shear strain detection. A silicone rubber layer, dyed with color inks, is used to quantify the shear magnitude of the sensing layer. This principle was validated using the NUSense camera-based tactile sensor. The wide-angle camera captures the elongation of the soft pad under mechanical load, a phenomenon attributed to the Poisson effect. The physical and optical properties of the inked pad are essential and should ideally remain stable over time. We tested the robustness of the sensor by subjecting the outermost layer to multiple load cycles using a robot arm. Additionally, we discussed potential applications of this sensor in force sensing and contact localization.

==> content/application.tex <==
\section{application}
\label{sec:appl}
This section shows how the NUSense can be used (TODO Tleukhan).

\begin{itemize}
    \item Force measure. Single point touch was calibrated using two intenders. Intender one was with the dome shape. Radius of the dome shape intender tip was 5 mm. Thus the area of contact was small.  It was used for calibration from 1 N to 3 N. Intender two was flat cylinder of radius 4 mm. The area of contact was larger than in the intender one. Intender two was used for calibration from 3 N to 8 N. Thus the applied preassure varied from XXXX to YYYY. Sensitiity (banana vs force) \textbf{EXPERIMENTS DONE}
    \item Hysteresis plot for the single point contact at 0.5 mm/sec. \textbf{EXPERIMENTS DONE}
    \item Robustness test for many cycling loads \textbf{TODO}
    \item Recovery test: cut the top layer. \textbf{TODO} 
    \item Two-point contact at distance of 20 mm, 30 mm, and 40 mm in between  \textbf{EXPERIMENTS DONE}
    \item EDGE experiments were not done. 
    \item Detect contact type Point and Edge type detection works. PCA will be applied.
    \item No shear forces.
    \item No Weight estimation without learning (gravity will help to estimate the mass)
    \item No Shape identification
    \item No area of contact (size) estimation
    \item No bandwidth experiments.
\end{itemize}


 







Spatial resolution (two closest points)









==> content/data_processing.tex <==
\section{NUSkin Data Processing}
\label{sec:data_proc}

In this section, we show how the raw image from the NUSense converted to useful information (TODO by Tleukhan).

Algorithm (by 30th of June coded up, 7th of july to write)

Pipeline

github link





\subsection{Background}


\subsubsection{B-Spline Surface}
\begin{figure}[h]
\centering
\includegraphics[width=0.2\textwidth]{figures_NUSense/bslpline_curve.png}
\caption{Example of bspline curve. Illustration of the elevated points, $u_0$ , $u_1$ , ... , $u_m$. P are the control points. Knot vector U = ( $u_0$ , $u_1$ , ... , $u_m$)}
\label{fig:bsplinecurve}
\end{figure} 


A B-spline surface (a collection of Bezier patches) is a tensor product surface of B-Spline curves. It is a parametric surface constructed using control points and B-spline basis functions. It is defined by two sets of basis functions, one for each parametric direction (u and v), and a set of control points arranged in a grid. A B-spline surface $\mathbf{S}(u, v)$ is defined as:

\begin{equation}
\mathbf{S}(u, v) = \sum_{i=0}^{n} \sum_{j=0}^{m} N_{i,p}(u) M_{j,q}(v) \mathbf{P}_{i,j}
\end{equation}

where:
\begin{itemize}
    \item $\mathbf{P}_{i,j}$ are the control points arranged in a grid.
    \item $N_{i,p}(u)$ are the B-spline basis functions of degree $p$ in the $u$-direction.
    \item $M_{j,q}(v)$ are the B-spline basis functions of degree $q$ in the $v$-direction.
    \item $n$ and $m$ are the number of control points in the $u$ and $v$ directions, respectively.
\end{itemize}

The B-spline basis functions $N_{i,p}(u)$ and $M_{j,q}(v)$ are defined recursively using the Cox-de Boor recursion formula.

\paragraph{Basis Functions for $u$-Direction}

For a given degree $p$ and knot vector $U = \{ u_0, u_1, \ldots, u_{n+p+1} \}$, the basis functions $N_{i,p}(u)$ are defined as:

\begin{enumerate}
    \item \textbf{Zero Degree Basis Functions:}
    \begin{equation}
    N_{i,0}(u) = 
    \begin{cases} 
    1 & \text{if } u_i \le u < u_{i+1} \\
    0 & \text{otherwise}
    \end{cases}
    \end{equation}

    \item \textbf{Recursive Definition:}
        \begin{align}
            N_{i,p}(u) &= \frac{u - u_i}{u_{i+p} - u_i} N_{i,p-1}(u) \nonumber \\
            &\quad + \frac{u_{i+p+1} - u}{u_{i+p+1} - u_{i+1}} N_{i+1,p-1}(u)
        \end{align}
\end{enumerate}

\paragraph{Basis Functions for $v$-Direction}
Similarly, for a given degree $q$ and knot vector $V = \{ v_0, v_1, \ldots, v_{m+q+1} \}$, the basis functions $M_{j,q}(v)$ are defined as:

\begin{enumerate}
    \item \textbf{Zero Degree Basis Functions:}
    \begin{equation}
    M_{j,0}(v) = 
    \begin{cases} 
    1 & \text{if } v_j \le v < v_{j+1} \\
    0 & \text{otherwise}
    \end{cases}
    \end{equation}

    \item \textbf{Recursive Definition:}
    \begin{align}
    M_{j,q}(v) &= \frac{v - v_j}{v_{j+q} - v_j} M_{j,q-1}(v) \nonumber \\
    &\quad + \frac{v_{j+q+1} - v}{v_{j+q+1} - v_{j+1}} M_{j+1,q-1}(v)
    \end{align}
\end{enumerate}

The B-spline surface is evaluated by computing the weighted sum of the control points, where the weights are the values of the basis functions at specific parameter values $u$ and $v$. The parameter values $u$ and $v$ vary between 0 and 1, and the evaluation typically involves a fine grid of $u$ and $v$ values to generate a smooth surface.

\subsubsection{Euclidean Distance}
The Euclidean distance is used to measure the straight-line distance between two points in Euclidean space. For two points $\mathbf{P}_1 = (x_1, y_1, z_1)$ and $\mathbf{P}_2 = (x_2, y_2, z_2)$, the Euclidean distance $d$ is given by:

\begin{equation}
d(\mathbf{P}_1, \mathbf{P}_2) = \sqrt{(x_2 - x_1)^2 + (y_2 - y_1)^2 + (z_2 - z_1)^2}
\end{equation}

The Euclidean distance is computed between corresponding evaluated points from two B-spline surfaces. The total Euclidean distance is the sum of distances for all pairs of corresponding points:

\begin{equation}
\text{Total Distance} = \sum_{i=1}^{N} d(\mathbf{P}_{1i}, \mathbf{P}_{2i})
\end{equation}

where $N$ is the number of evaluated points on the B-spline surface.

As final steps, a binary image is created based on the Euclidean distances. Pixels with distances greater than a threshold are set to white, and others are set to black. The binary image undergoes dilation to combine close white regions. Connected component analysis is applied to isolate the largest connected component, which is then used for shape detection. Contours are detected in the largest connected component (Fig.~\ref{fig:largest_connected_comp}). Each contour is classified based on geometric properties (area, aspect ratio, extent). The orientation angle of each shape is calculated using image moments. 

\begin{figure}[h]
\centering
\includegraphics[width=0.1\textwidth]{figures_NUSense/largest_connected_component.png}
\caption{Binary Image with Largest Connected Component}
\label{fig:largest_connected_comp}
\end{figure} 

\subsection{The Algorithm Pipeline}
%[Madina]:could be just, the algorithm uses Opencv and Numpy libraries. We start with the fisheye image accepted from the camera. 
The algorithm begins by importing OpenCV and NumPy libraries, followed by loading the fish eye image. A camera matrix and distortion coefficients are defined to model the fisheye lens characteristics. Using these parameters, a new camera matrix is estimated to undistort and rectify the image. Undistort rectify maps are then initialized, and these maps are applied to the original image to produce the undistorted image. This process effectively removes the fisheye distortion, resulting in a geometrically accurate image. The resulting image is then processed to detect and highlight quadrilaterals using several image processing techniques.

Initially, a region of interest (ROI) within the image is specified by the coordinates and dimensions (x, y, width, height). This ROI is extracted from the original image and converted to a grayscale image for further processing. Contrast Limited Adaptive Histogram Equalization (CLAHE) is applied to the grayscale image to enhance its contrast. CLAHE improves the visibility of features by equalizing the histogram of local regions. Next, a bilateral filter is applied to the enhanced grayscale image to reduce noise while preserving edges, which are then detected using the Sobel filter. The combined Sobel image is thresholded to create a binary image. This binary image undergoes morphological operations, specifically dilation followed by erosion (closing), to fill small gaps and remove noise. These operations help in creating more solid shapes for contour detection. Contours are detected in the processed binary image using \textbf{cv2.findContours()}. Each contour is approximated to a polygon, and those with four vertices are identified as quadrilaterals. Additional filters based on area, solidity, and convex hull are applied to ensure the detected quadrilaterals are significant and accurate. The algorithm then connects the corners of the detected quadrilaterals that are within a specified distance threshold. It draws lines between the closest points of different quadrilaterals. Midpoints of these lines are calculated, and small circles are drawn at these midpoints to highlight connections. The results can be seen in Fig.~\ref{fig:Pressure_2}.

\begin{figure}[h]
\centering
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures_NUSense/Pressure_2_defisheyed.jpg}
    \caption{Input image (under pin pressure)}
    \label{fig:Pressure_2}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures_NUSense/Pressure_2_output.jpg}
    \caption{Processed image with detected quadrilaterals}
    \label{fig:Pressure_2_output}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.1\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures_NUSense/blue_dots.png}
    \caption{Magnified view. Blue - the control points.}
    \label{fig:blue_dots}
\end{subfigure}
\caption{Evaluated Points from Images}
\label{fig:Pressure_2}
\end{figure}

The next step starts by loading an image and converting it to the Hue-Saturation-Value (HSV) color space to isolate the blue color range. Contours of the blue regions are identified, and the centroids of these contours are computed and stored as control points. These control points are then sorted and arranged into a grid to form a B-spline surface~\cite{bspline}. The surface is evaluated to obtain a set of points, which are then used for further analysis (Fig.~\ref{fig:control_points}). 

\begin{figure}[h]
\centering
\begin{subfigure}[b]{0.2\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures_NUSense/control_points_image1.png}
    \caption{Evaluated Points (without deformations)}
    \label{fig:control_points_1}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.2\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures_NUSense/control_points_image2.png}
    \caption{Evaluated Points (with deformations)}
    \label{fig:control_points_2}
\end{subfigure}
\caption{Evaluated Points from Images}
\label{fig:control_points}
\end{figure}

The algorithm processes two images, evaluates the Euclidean distances between corresponding points on the B-spline surfaces of the two images, and sums these distances to quantify differences. It visualizes the Euclidean distances and control points through scatter plots, highlighting the differences between the images(Fig.~\ref{fig:euclidean_distances}). 

\begin{figure}[h]
\centering
\includegraphics[width=0.2\textwidth]{figures_NUSense/euclidean_distances.png}
\caption{Euclidean Distances Between Evaluated Points}
\label{fig:euclidean_distances}
\end{figure} 




%%%%%%%%%%REMOVED%%.%%%WE%%DID%%NOT%%%DO%%%HEAR%%%.%%%%%%%%%%%%%%%%%%%%%
%\subsubsection{Shear and Torsional Deformations}
% When the sensing layer laterally shifts from its resting state so that its length does not change, the color of a particular pixel, that was at the border between yellow and red regions of the pattern during the resting state, changes from yellow to red or vice versa depending on direction because the piece of the colored pattern  shifts. This shift happens when the sensing surface is under the load with a normal force applied to the entire surface $F_z$ and a tangential force $F_x$ or $F_y$ due to the static friction force between the sensor and an object in contact. The magnitude of the tangential force is equal to the magnitude of the friction force that is proportional to the static friction coefficient between the interacting surfaces. Figure~\ref{fig:concept} exemplifies the change of the color spectra of light from yellow to red due to mechanical load that changes from $F_x = 0$  to $F_x \neq 0$ as shown in Fig.~\ref{fig:concept}. 

% Shifting  from  yellow  to  red (and vice versa) can also occur  when the patterned layer twists in the planar surface. The pattern is made as a chessboard. The twisting and shear deformations cause different  shape changes in such color pattern seen by the camera. Specifically, the center of the colored pattern shifts during shear deformation, but it remains the same while twisting. The twisting deformation happens when the sensing surface is under the load with a normal force applied to the entire surface and torque $T$ applied to the upper side of the cylinder (Fig.~\ref{fig:concept}).

==> content/properties.tex <==
\section{NUSkin Properties}
\label{sec:properties}

In this section, we discuss/measure the sensor properties such as
\begin{enumerate}
    \item \textbf{Bandwidth} - the sensor's ability to respond to instantaneous changes in the physical conditions being measured, i.e find the highest frequency the sensor can measure. TAS NOTE: I do not think we need to do this since it is not very important thing for optical sensors.
    \item \textbf{Sensitivity} - this is doable. Need to come up with nice experiment to do it. TODO by Madina and Tleukhan.
    \item \textbf{Repeatability} - must be done. TODO by Madina and Tony.
    \item \textbf{Spatial resolution} - I am not sure about this?
    \item \textbf{Hysteresis} - ability to recover after pressure released
\end{enumerate}
